UniCtrl: Improving the Spatiotemporal Consistency of Text-to-Video Diffusion Models via Training-Free Unified Attention Control

Video Diffusion Models have been developed for video generation, usually integrating text and image conditioning to enhance control over the generated content. Despite the progress, ensuring consistency across frames remains a challenge, particularly when using text prompts as control conditions. To address this problem, we introduce UniCtrl, a novel, plug-and-play method that is universally applicable to improve the spatiotemporal consistency and motion diversity of videos generated by text-to-video models without additional training. UniCtrl ensures semantic consistency across different frames through cross-frame self-attention control, and meanwhile, enhances the motion quality and spatiotemporal consistency through motion injection and spatiotemporal synchronization. Our experimental results demonstrate UniCtrl's efficacy in enhancing various text-to-video models, confirming its effectiveness and universality.

==> fig/motion_degree.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/src/Motion_Injection_Degree.pdf}
    %\vspace*{-20pt}
    \caption{In our framework, we use key and value from the first frame as represented by $K^0$ and $V^0$ in the self-attention block. We also use another branch to keep the motion query $Q_\textrm{m}$ for motion control. At the beginning of every sampling step, we let the motion latent equal to the sampling latent, to avoid spatial-temporal inconsistency. We explain details of our framework in Algorithm \ref{alg:selfattn} and Algorithm \ref{alg:motion_injection_degree}.}
    \label{fig:motion_injection_degree}
\end{figure*}
